ChartMimic: Evaluating LMM's Cross-Modal Reasoning Capability via Chart-to-Code Generation

We introduce a new benchmark, ChartMimic, aimed at assessing the visually-grounded code generation capabilities of large multimodal models (LMMs). ChartMimic utilizes information-intensive visual charts and textual instructions as inputs, requiring LMMs to generate the corresponding code for chart rendering. ChartMimic includes 4,800 human-curated (figure, instruction, code) triplets, which represent the authentic chart use cases found in scientific papers across various domains (e.g., Physics, Computer Science, Economics, etc). These charts span 18 regular types and 4 advanced types, diversifying into 201 subcategories. Furthermore, we propose multi-level evaluation metrics to provide an automatic and thorough assessment of the output code and the rendered charts. Unlike existing code generation benchmarks, ChartMimic places emphasis on evaluating LMMs' capacity to harmonize a blend of cognitive capabilities, encompassing visual understanding, code generation, and cross-modal reasoning. The evaluation of $3$ proprietary models and 14 open-weight models highlights the substantial challenges posed by ChartMimic. Even the advanced GPT-4o, InternVL2-Llama3-76B only achieved an average score across Direct Mimic and Customized Mimic tasks of 82.2 and 61.6, respectively, indicating significant room for improvement. We anticipate that ChartMimic will inspire the development of LMMs, advancing the pursuit of artificial general intelligence.

==> prompts/code.tex <==
% \begin{figure}[H]
% \begin{tcolorbox}[colback=white, colframe=black, title=Code example for Heatmap\_20]
% \# ===================

% \# Part 1: Importing Libraries

% \# ===================

% import matplotlib.pyplot as plt

% import pandas as pd

% \# ===================
% \# Part 2: Data Preparation
% \# ===================
% \# Define the emotion labels
% emotions = [\\
%     "angry",\\
%     "sad",\\
%     "disgust",\\
%     "contempt",\\
%     "fear",\\
%     "neutral",\\
%     "surprise",\\
%     "happy",\\
% ]

% \# Define the data for the original and adjusted values
% original_values = [0.10, 0.00, 0.30, 0.00, 0.00, 0.50, 0.00, 0.10]
% adjusted_values = [0.12, 0.00, 0.44, 0.00, 0.00, 0.44, 0.00, 0.00]
% titles = ["Original", "Adjusted"]

% \# ===================
% \# Part 3: Plot Configuration and Rendering
% \# ===================
% \# Create a figure with two subplots (one for original and one for adjusted values)
% fig, (ax1, ax2) = plt.subplots(2, 1, figsize=(10, 8))

% \# Define the color palette
% cmap = plt.get_cmap("coolwarm")

% \# Plot heatmap for original values
% im1 = ax1.imshow(pd.DataFrame([original_values], columns=emotions), cmap=cmap)
% ax1.set_title(titles[0])
% ax1.set_xticks(range(len(emotions)))
% ax1.set_xticklabels(emotions, rotation=45, ha="center")
% ax1.set_yticks(range(1))
% ax1.set_yticklabels([""], rotation=0)

% \# Add annotations for original values
% for i in range(1):
%     for j in range(len(emotions)):
%         ax1.text(
%             j, i, f"{original_values[j]:.2f}", ha="center", va="center", color="black"
%         )

% \# Plot heatmap for adjusted values
% im2 = ax2.imshow(pd.DataFrame([adjusted_values], columns=emotions), cmap=cmap)
% ax2.set_title(titles[1])
% ax2.set_xticks(range(len(emotions)))
% ax2.set_xticklabels(emotions, rotation=45, ha="center")
% ax2.set_yticks(range(1))
% ax2.set_yticklabels([""], rotation=0)

% \# Add annotations for adjusted values
% for i in range(1):
%     for j in range(len(emotions)):
%         ax2.text(
%             j, i, f"{adjusted_values[j]:.2f}", ha="center", va="center", color="black"
%         )

% \# Display the figure
% plt.subplots_adjust(hspace=-0.5)

% \# ===================
% \# Part 4: Saving Output
% \# ===================
% plt.tight_layout()
% plt.savefig("heatmap_20.pdf", bbox_inches="tight")

% \end{tcolorbox}
% \caption{Code example for Heatmap\_20.}
% \label{fig:code}
% \end{figure}

==> prompts/human_evaluation.tex <==
\begin{figure}[th]
\begin{tcolorbox}[colback=white, colframe=black, title=Instruction for Human Evaluation]
1. Chart Type (20 points)
\\
Does the generated image contain all chart types present in the original image (e.g., line chart, bar chart, etc.)?
\\
\\
2. Image Layout (10 points)
\\
Is the arrangement of subplots in the generated image consistent with the original (e.g., number of rows and columns)?
\\
\\
3. Textual Content (20 points)
\\
Does the generated image include all textual elements from the original image (e.g., title, annotations, axis labels, etc.), excluding the axis tick labels?
\\
\\
4. Data (20 points)
\\
Does the data trend in the generated image closely resemble that of the original image?
\\
\\
5. Style (20 points)
\\
Are the colors (line colors, fill colors, etc.), marker types (shape of points, line styles, etc.), legends, grids, and other details in the generated chart similar to those in the original?
\\
\\
6. Clarity (10 points)
\\
Is the generated chart clear and free from overlap?
\\
\\
Each of these six points has a corresponding maximum score. Based on the condition of the generated chart, score each point accordingly to arrive at a total score.
\end{tcolorbox}
\label{fig:prompt_human_evaluation}
\caption{Instruction for Human Evaluation.}
\end{figure}

==> sections/checklist.tex <==
\newpage
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} The main claims made in the abstract and introduction accurately reflect the paper's contributions and scope. 
  \item Did you describe the limitations of your work?
    \answerYes{} We describe the limitations of on our work in \cref{ss:conclusions}.
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} Our work focuses on scientific charts, thus there is almost no negative societal impacts. However, we still explain this in the supplemental material.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{} We have read them and ensure to conforms to them.
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{We do not include theoretical results.}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{We do not include theoretical results.}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} We include the code, data, and instructions needed to reproduce the main experimental results in the supplemental material.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{} Our work does not take training of the models.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} We calculate the p-value for the correlation between human evaluation and automation metrics in~\cref{ss:human_evaluation}.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{} Our work does not take training of the models; we pay attention to inference and evaluation.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} Our charts have been manually redrawn at the end, and any corresponding reference data~(all with CC BY 4.0 license) that may exist will be explained in the supplement.
  \item Did you mention the license of the assets?
    \answerYes{} We mention the potential license of the assets in the supplemental material.
    % ~\cref{ss:data_annotation}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{} We include new assets in the supplemental material. We make it for CC BY 4.0 license.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{} Our reference figures are all CC BY 4.0 licenses.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{} Our benchmark focuses on scientific charts, we have checked the data during annotation and there are no such issues.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{} We include them in the supplemental material.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{} Our benchmark focuses on scientific charts, and there are no such issues.
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{} Our benchmark is standardized by the paper's authors and volunteer graduate students, while human evaluations are evaluated by volunteer university students and graduate students as detailed in the supplemental material.
\end{enumerate}

\end{enumerate}

==> tables/error_analysis.tex <==
\begin{table}[]
\centering
\begin{tabular}{c|ccc}
\toprule
\multicolumn{1}{c|}{\textbf{Low-level Aspect}} & \multicolumn{3}{c}{\textbf{Error Category Statistics}}                               \\
\midrule
\multirow{2}{*}{ChartType}           & Confusion               & Missing                 & Hallucination           \\
\cmidrule(lr){2-4}
                                     & \multicolumn{1}{c}{87}  & \multicolumn{1}{c}{99}  & \multicolumn{1}{c}{26}  \\
\midrule
\multirow{2}{*}{Text}                & Confusion               & Missing                 & Hallucination           \\
\cmidrule(lr){2-4}
                                     & \multicolumn{1}{c}{50}  & \multicolumn{1}{c}{115} & \multicolumn{1}{c}{121} \\
\midrule
\multirow{2}{*}{Color}               & Similar Color           & \multicolumn{2}{c}{Definitely Different}          \\
\cmidrule(lr){2-4}
                                     & \multicolumn{1}{c}{247} & \multicolumn{2}{c}{120} \\
\bottomrule
\end{tabular}
\caption{}
\label{tab:error_analysis}
\end{table}

==> tables/tableprompt.tex <==
\begin{wraptable}{r}{0.45\textwidth}
    \vspace{-1.4em}
    \centering
    \small
    \caption{Results for different prompting methods on GPT-4o on \tasknameone{} task.}
    \vspace{-0.7em}
    \label{tab:different_prompt_results}
    \setlength{\tabcolsep}{2.2pt}
    \resizebox{\linewidth}{!}{\begin{tabular}{c|cccccc|c|c}
    \toprule
    \multirow{2.4}{*}{Model} & \multirow{2.4}{*}{\shortstack{Exec.\\Rate}} & \multicolumn{5}{c|}{Low-Level} & \multicolumn{1}{c|}{High-Level} & \multirow{2.4}{*}{Overall} \\
    \cmidrule{3-8} 
      & & Text & Layout   & Type   & Color    & Avg.  & GPT-4V  &  \\
    \midrule
    Direct & 93.3 & 81.7 & 90.1 & 77.6 & 67.6 & 79.3 & 83.7 & 81.5 \\
    HintEnhanced & 92.2 & 78.3 & 86.8 & 75.5 & 65.0 & 76.4 & 83.3 & 79.8 \\
    \gr SelfRevision & 96.9 & 84.4 & 92.3 & 85.4 & 72.3 & 83.6 & 88.2 & 85.9 \\
    Scaffold& 94.3 & 80.2 & 88.5 & 74.0 & 63.0 & 76.4 & 80.7 & 78.6\\
    \bottomrule
    \end{tabular}}
    \vspace{-1.1em}
\end{wraptable}

